DB4HLS: A Database of High-Level Synthesis Design Space Explorations

High-Level Synthesis (HLS) frameworks allow to easily specify a large number of variants of the same hardware design by only acting on optimization directives. Nonetheless, the hardware synthesis of implementations for all possible combinations of directive values is impractical even for simple designs. Addressing this shortcoming, many HLS Design Space Exploration (DSE) strategies have been proposed to devise directive settings leading to high-quality implementations while limiting the number of synthesis runs. All these works require considerable efforts to validate the proposed strategies and/or to build the knowledge base employed to tune abstract models, as both tasks mandate the syntheses of large collections of implementations. Currently, such data gathering is performed ad-hoc, a) leading to a lack of standardization, hampering comparisons between DSE alternatives, and b) posing a very high burden to researchers willing to develop novel DSE strategies. Against this backdrop, we here introduce DB4HLS, a database of exhaustive HLS explorations comprising more than 100000 design points collected over 4 years of synthesis time. The open structure of DB4HLS allows the incremental integration of new DSEs, which can be easily defined with a dedicated domain-specific language. We think that of our database, available at https://www.db4hls.inf.usi.ch/, will be a valuable tool for the research community investigating automated strategies for the optimization of HLS-based hardware designs.

==> DB4HLS_ A Database of High-Level Synthesis Design Space Explorations/content.tex <==
% As a general rule, do not put math, special symbols or citations
% in the abstract or keywords.
\begin{abstract}


High-Level Synthesis (HLS) frameworks allow to easily specify a large number of variants of the same hardware design by only acting on optimization directives. Nonetheless, the hardware synthesis of implementations for all possible combinations of directive values is impractical even for simple designs. Addressing this shortcoming, many HLS Design Space Exploration (DSE) strategies have been proposed to devise directive settings leading to high-quality implementations while limiting the number of synthesis runs. All these works require considerable efforts to validate the proposed strategies and/or to build the knowledge base employed to tune abstract models, as both tasks mandate the syntheses of large collections of implementations. Currently, such data gathering is performed ad-hoc, a) leading to a lack of standardization, hampering comparisons between DSE alternatives, and b) posing a very high burden to researchers willing to develop novel DSE strategies. Against this backdrop, we here introduce DB4HLS, a database of exhaustive HLS explorations comprising more than 100000 design points collected over 4 years of synthesis time. The open structure of DB4HLS allows the incremental integration of new DSEs, which can be easily defined with a dedicated domain-specific language.  
We think that of our database, available at \small{\texttt{https://www.inf.usi.ch/phd/ferretti/db4hls.html}}, will be
%extremely compelling 
%LP: maybe a bit too strong....
a valuable tool 
for the research community investigating automated strategies for the optimization of HLS-based hardware designs.

%High-Level Synthesis (HLS) tools allow the generation of a large variety of hardware implementations from the same specification by setting different optimization directives.
%While one hand  HLS design flows allow designers to easily explore different design alternative, they also require  strategies able to navigate the vast design space of microarchitectural alternatives to identify the most promising implementations while minimising the number of time-consuming HLS runs.
%It allows fast exploration of different design alternatives. 
%In the past years many research efforts have lead to different strategies aiming at identifying the most promising implementations while minimising the number of time-consuming HLS runs.
%Despite the many publication, the evaluation of such methodologies lacks in standardisation. Moreover, recently published works are showcasing the importance, for such methodologies, to rely on large datasets to build accurate models. Due to the long time required to generate such data, there is scarcity of such resources.
%We preset DB4HLS, a collection of HLS implementations gathered targeting the Machsuite benchmarks and a framework to expand the database. Our contributions aim at offering researchers the possibility to standardize the evaluation process of existing methodologies and an important source of data for ML-based approaches.
 
\end{abstract}

% Note that keywords are not normally used for peerreview papers.
\begin{IEEEkeywords}
High-Level Synthesis, Databases, Machine Learning, Big Data, Design Space Exploration.
\end{IEEEkeywords}

\section{Introduction}

High-Level Synthesis (HLS) fostered a revolution in hardware design. HLS frameworks allow the specification of hardware components in languages such as C, C++, or SystemC. As opposed to traditional Register Transfer Level (RTL) approaches, HLS flows do not require detailed descriptions of the logic gates, memory elements and interconnects comprising hardware implementations. Instead, these are automatically generated, based on the high-level specifications and on a set of directive values specifying optimizations such as the unrolling factor of loops and the inlining of functions. By decoupling specification from implementation, HLS allows unprecedented productivity, leading to considerable reductions in non-recurring engineering costs.

Nonetheless, while HLS allows to easily define vast design spaces for a given hardware specification, determining the performance (latency) and resource requirements (area, power) of each implementation still requires time-consuming syntheses. The amount of possible implementations of a design explodes exponentially with the number of applied directives, while, in general, only a few of them are Pareto-optimal from a performance/resources perspective. Exhaustive explorations are therefore wasteful (since only Pareto implementations are of interest) and impractical beyond very simple cases. 

Various strategies, which we summarize in Section \ref{sec:SoA}, have been proposed to identify (or approximate) the set of Pareto-implementations while minimising the number of synthesis runs \cite{LiuJun13} \cite{FerrettiJan18} \cite{ferretti2018lattice}. This problem is named \emph{HLS-driven Design Space Exploration (DSE)}. The proposed DSEs strategies are typically validated against exhaustive explorations, which the authors performed ad-hoc. Moreover, works such as \cite{wang20Mar} \cite{Ferretti20Oct} rely on prior knowledge to steer the HLS exploration process. 
Performing the huge number of synthesis required for validation or for generating a high-quality knowledge base entails a very high effort, which at present must be repeated ex-novo when investigating the performance of a novel DSE methodology. 

Against this backdrop, we introduce DB4HLS, a database of high-level synthesis design space explorations. The database comprises more than 100000 design points, reporting the synthesis outcomes of exhaustive explorations performed on 39 designs from the MachSuite \cite{reagen2014machsuite} benchmark suite. In addition, we define a simple domain-specific language to define design spaces, resulting in an open infrastructure that can be enriched by further contributions from the research community.

We believe that, by providing standardized synthesis data sets, our effort will allow easier comparisons among DSE strategies, enabling fairer evaluations of the strengths and weaknesses of each approach. It will also facilitate the development and assessment of future design exploration frameworks, spurring research in this challenging field.


%HLS tools enables rapid and the automatic specification of hardware designs from high-level specifications given, for example, as C/C++ or SystemC code. Conversely, the generation of the corresponding hardware implementation is still a time consuming process that can't be avoided. 
%The HLS design flow allows designers to specify functionalities at a higher level of abstraction than register-transfer level (RTL), and to guide the synthesis process to generate different micro-architectural implementations by applying optimsation directives to the original specifications.
%By choosing different set of the HLS directives, designers can influence the resulting performance and costs of the synthesised implementations, enabling the rapid exploration of the design space with respect to conflicting objectives such as performance (latency) and cost (area, power).
%%Examples of directives include the unrolling factor of a loop, the inlining of functions, and the mapping of arrays to memory structures. 
%%HLS enable the rapid exploration of the design space with respect to conflicting objectives such as performance (latency, throughput) and cost (area, power)~\cite{liu_date12}.
%However, due to the large number of implementations resulting from the combination of the different directives and the difficulties to foresee and quantify the effect of those before the execution of the synthesis process, exhaustive exploration is often infeasible. In fact, the number of different implementations increases exponentially with the number of considered directives, thus making exhaustive exploration impossible even for simple cases.
% Moreover, the synthesis is a time-consuming process which is often traded-off by designer with r
%In addition the synthesis is a time-consuming process that often forces the designers to trade off the quality of the design exploration with the time required for it. The process of identifying the most effective implementations, from a cost and performance perspective, while minimising the number of synthesis runs is named \emph{HLS-driven design-space exploration (DSE)}.

%This work provides researchers with a set of already performed design space explorations (DSE) targeting functions of the MachSuite \cite{reagen2014machsuite} benchmark suite.

%%The identification of the most effective implementation, from a cost and performance perspective, while minimising the number of synthesis runs is named \emph{HLS-driven design-space exploration (DSE)}. 
%Figure \ref{fig::motivation} illustrates HLS design flows and the result of applying different directives to a specification.

\section{Related Works}

\label{sec:SoA}

%To tackle this problem researchers have proposed different strategies. 
State of the art DSE frameworks for HLS follow three main approaches. Black-box methodologies aim, after an initial phase, at iteratively refining explorations by smartly selecting additional design points. To this end, they employ unsupervised learning strategies such as clustering \cite{FerrettiJan18}, random forest \cite{LiuJun13}, lattice traversing \cite{ferretti2018lattice} and response surface models \cite{XydisOct14}.
Model-based strategies, on the other hand, estimate performance and resource requirements of implementations by developing an analytical formulation of the effect of directives when applied to a design. Typically, they can well approximate the Pareto set of best-performing implementations with few synthesis, but are restricted in the type of targeted optimizations (e.g., loop unrolling and dataflow in \cite{ZhongDec14}).
The authors of all these works adopt as figure of merit either the Hypervolume or the Average Distance from Reference Set (ADRS) for validation, and both require the computation of true Pareto frontiers from exhaustive explorations.
Recently, a promising research avenue has focused instead on exploring prior knowledge to reduce the complexity of DSE problems in hardware design. These works \cite{wang20Mar} \cite{Ferretti20Oct} leverage the availability of a comprehensive knowledge base, such as the one we describe in our paper, to achieve exploration results close to that of model-based strategies while being much more flexible in the number and type of supported directives.

%In the past years, researchers have proposed different DSE strategies. Model based approaches \cite{} \cite{} \cite{} estimate performance and resources utilisations of a set of optimizations, given an analytical or a learning-based model of the synthesis tool. Alternatively, refinement-based strategies \cite{} \cite{} \cite{} build their knowledge relying on the outcome of the synthesis process and they build the underlying model online, during the DSE.
%Both of these approaches usually need an initial source of data to  build their knowledge. The generation of this initial knowledge base requires the execution of time consuming synthesis-runs and is usually built ex-novo by researchers presenting new methodologies.

%Recently, Doppa et al. \cite{DoppaOct19} highlighted the importance of leveraging prior knowledge to effectively reduce the complexity of DSE problems. A small number of works take this stance in the context of hardware design.
%In \cite{DaiApr18} the authors aim at improving the accuracy of HLS estimations using post-synthesis data; in \cite{liuJun19} the goal is to estimate the performance on FPGA from an ASIC synthesis report; while \cite{DeshwalOct19} leverages prior knowledge in the context of network-on-chip DSEs, to identify promising starting point for their exploration methodology.
%Finally, two recent works have proposed to leverage prior knowledge from a database of past exploration in order to steer the design space exploration of HLS design \cite{} \cite{} showcasing promising results while exploiting previous knowledge. All these works share a common aspect: they \emph{all require an initial knowledge base}.

%Finally, two recent works have proposed to leverage prior knowledge from a database of past exploration in order to steer the design space exploration of HLS design \cite{} \cite{} showcasing promising results while exploiting previous knowledge. All these works share a common aspect: they \emph{all require an initial knowledge base}.


%To tackle this problem, researchers have proposed different strategies, discussed in Section \ref{sec:SoA}, however, a fair comparison among those is often hard to perform. The main reasons are due to the fact that while some methodologies are agonistic to the number of directives, some others present restrictions on the directive considered.
%One of the reason of such difficulties is the fact that some strategies are specific for only few directives while other do not impose any restriction on the number of directive considered. 
%In addition to the need of knowledge to build reliable model, also a standardisation of the evaluation process across the different methodologies is a problem. In fact, in order to deal with treatable DSEs designers often constraint the design spaces according to different heuristics. Therefore, for a single design many different configuration space can be defined according to the designer pruning choices. Hence, reproducing experiments across different methodologies, and evaluate qualitatively them may be difficult since different experimental setups may have an impact on the resulting quality of the DSE methodologies.

While benchmark suites dedicated to hardware design are available, such as CHStone \cite{hara2008chstone}, MachSuite \cite{reagen2014machsuite}, Rosetta \cite{zhou2018rosetta} and S2CBench \cite{schafer2014s2cbench}, they only provide specifications (in the form C/C++ code) as benchmarks. Conversely, our DB4HLS suite offers rich and well-defined design spaces and related synthesis outcomes, greatly easing the burden of performing comparative evaluations of exploration methodologies.
To the best of our knowledge, this is the first database of HLS implementation made publicly available with the intent of standardize the evaluation process, and provide a source of knowledge for ML strategies.
%LP: I think that adding the above sentence would be good, here.

%In the past years, many research effort have been conducted to provide sets of applications representing good candidates for the HLS design flow. Different benchmark suites have been published, such as CHStone \cite{hara2008chstone}, MachSuite \cite{reagen2014machsuite}, Rosetta \cite{zhou2018rosetta} and S2CBench \cite{schafer2014s2cbench} offering different applications amenable for hardware accelerators.
% but, to the best of our knowledge, no dataset providing already synthesised implementations exploitable from DSE methodologies have been published.
%These benchmarks have often been target of DSE methodologies \cite{FerrettiJan18}, \cite{ferretti2018lattice} \cite{} and different exploration have been performed over the available designs to evaluate the effectiveness of such strategies. While on the one hand, these benchmarks offer the opportunity to evaluate the methodologies over the same set of applications, the evaluation of them across a set of well defined, and easy to reproduce DSE is rarely achievable.

%In addition, recent works have showcased how leveraging prior knowledge from different explorations may improve the quality of DSEs. Machine Learning (ML), Transfer Learning (TL) and Deep Learning (DL) approaches are viable choices for such scenario, however, these methodologies usually rely on a large quantity of data in order to build a model. The lack of data, and the difficulties to build reliable models without a large training dataset has often limited the use of ML approaches with respect to other fields. Build such knowledge requires a large amount of time due to the time-consuming synthesis process. This factor became the barrier of entrance for new ML-based approaches.

%\begin{figure}[t]
%\centering
%\includegraphics[width=\linewidth]{imgs/motivation}
%\caption{HLS design flow. Starting from high level specifications the HLS process generates different implementations according to the set of HLS directive specified}
%\label{fig::motivation}
%\vskip -2em
%\end{figure}
%Given this situation, it is clear that while benchmarks of HLS designs and DSE methodologies have been investigated, no datasets of reusable knowledge both for evaluation and training of new methodologies exists. 
%In this work \emph{we aim at providing a database of HLS implementations offering a reliable source of data to target DSE problems}. The contribution offered by the database is three fold: a) a database of design space exploration, b) a domain-specific language used to describe a configuration space for a target design, c) an interface to generates new explorations and increase the database.
%To the best of our knowledge, this will be the the first publicly available database of already synthesised implementations to be published.

%Figure~\ref{fig:motivation} illustrates our approach. When exploring a new \emph{target} design with HLS, we first select a \emph{source} design from a library of previously completed explorations. The source design is the one whose specification is most similar to the target one. Then, we consider the combinations of directives that led to the best results for the source design. These are Pareto-optimal implementations (marked with red crosses in Figure \ref{fig:intro}), i.e. those for which no other implementations resulted in both less area and lower latency. 
%The main idea is that the similarity among the two designs justify the translation of the directives from the source design into directives for the target design, in order to lead the search for an approximation of the set of Pareto-optimal target implementations. 



%\section{Related Works}

%\label{sec:SoA}

%Recent works proposing strategies to navigate HLS design-spaces can be  organized in two main categories. On one hand, model-based approaches \cite{ZhongDec14}
%\cite{PhamMar15} \cite{ZhongJun16} \cite{ZhaoOct17} rely on an estimation of performance and resource requirement of a given optimization. While mandating very few synthesis runs, such strategies struggle when coping with multiple, interdependent optimizations. Hence, they are often limited to capturing the effect of only few directives. 
%
%On the other hand, refinement-based frameworks rely on the outcome of some synthesis runs as a starting point, and aim to improve on this initial solution using different strategies such as random forest \cite{LiuJun13}, genetic algorithms \cite{SchaferMay12}, clustering \cite{FerrettiJan18} or local search techniques \cite{ferretti2018lattice}. Refinement-based methods are agnostic to the set of considered directives, but usually exhibit a slower convergence rate, because they must incrementally build a knowledge of the  design space being explored.



%Moreover, in a recent editor's note, Doppa et al. \cite{DoppaOct19} highlighted the importance of leveraging prior knowledge to effectively reduce the complexity of DSE problems. A small number of works take this stance in the context of hardware design.
%In \cite{DaiApr18} the authors aim at improving the accuracy of HLS estimations using post-synthesis data; in \cite{liuJun19} the goal is to estimate the performance on FPGA from an ASIC synthesis report; while \cite{DeshwalOct19} leverages prior knowledge in the context of network-on-chip DSEs, to identify promising starting point for their exploration methodology.
%Finally, two recent works have proposed to leverage prior knowledge from a database of past exploration in order to steer the design space exploration of HLS design \cite{} \cite{} showcasing promising results while exploiting previous knowledge.

%Given these research trends, a pice is missing. In fact, while benchmarks of HLS designs and DSE methodologies have been investigated, no datasets of reusable knowledge both for evaluation and training of new methodologies exists. To the best of our knowledge, this will be the the first publicly available database of already synthesised implementations to be published.

%Finally, Martins et al. \cite{MartinsApr16} also present a strategy to harness prior knowledge based on a similarity metric, but their framework is geared towards the selection of \emph{compiler} optimizations, as opposed to targeting the hardware domain of HLS.


%\section{Terminology}\label{sec:terminology}
%In this section we describe the terminology adopted in the paper and all the elements leading to the definition of design space from the DB4HLS perspective. In fact, the terminology introduced here reflects the construction of the database described in section \ref{fig::infrastructure}.

%%A \emph{benchmark} is a collection of software \emph{applications} implementing a functionality. Each application functionality may be realised in software in different ways. An instance of an application functionality is named \emph{algorithm}.
%A \emph{benchmark} is a software implementing a functionality. Each benchmark functionality may be realised in software in different ways. An instance of benchmark functionality is named \emph{algorithm}.

%Moreover, each algorithm may be specified differently; a specific version of an algorithm, synthesizable from HLS tools, is named \emph{HLS design} (or \emph{design}). A \emph{specification} is a high-level description of the design in a programming language such as SystemC or C/C++, given in input to the HLS tool. For each design one or more \emph{configuration spaces} can be defined and a configurations space defines all the different microarchitectural variations of a design to implement in hardware. 
%A \emph{configuration} is an element of the configuration space characterising a microarchitectural choice.

%An \emph{implementation} of a design is the output of a run of the HLS tool for a given configuration -- typically an automatically generated RTL code written in Verilog or VHDL.
%Each implementation is characterised by the values of a performance metric and a cost metric. 

%A \emph{synthesis configuration} (or, simply, \emph{configuration}) defines the transformations that a design undergoes through HLS. A designer controls these transformations with constraint and optimization \emph{directives}, such as loop unrolling or pipelining, array manipulation, and other control and datapath optimizations.
%A directive is associated with a \emph{location} in the code specification. A location could be either a label in the code or a language construct; for example, a loop or an array declaration.
%A designer can further customise some directives by specifying the \emph{values} for the directive parameters; for example, the designer can customise the amount of parallelism in the implementation by unrolling a loop a certain number of times or by setting a certain initiation interval for the pipeline implementing the loop. 
%The tuple comprising a type of directives, the location, and selected parameter values that the designer considers for the DSE task is named \emph{knob}.

%Figure \ref{fig::terminology} highlights the terminology and the differences between configuration, knob, location, directive, knob type, and knob values.
%To summarize, for each location, a designer can choose one or more directives and assign their parameter values.

%Finally, a \emph{design space} is the set of all the possible design configurations of the \emph{configuration space} and the corresponding \emph{implementations}.

%\begin{figure}[!t]
%	\centering
%	\includegraphics[width=\linewidth]{imgs/terminology-crop.pdf}
%	\caption{Representation of the terminology adopted in the paper. (left) The table proposes examples of knobs and their tuple indicating the knobs location, type and having different sets of values. (right) Example of configuration characterized by different knobs and their associated knob values.}
%	\label{fig::terminology}
%%\vskip -1em
%\end{figure}

\begin{table}[!tb]
% \footnotesize 
% \tiny
\centering
% \title{DNA source code encoding}
\caption{\small List of functions explored from MachSuite\cite{reagen2014machsuite}, grouped by benchmark. The table reports: benchmark name, function name, and size of the configuration space ($|CS|$).}
\label{table:functions}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|l|}
% \hline
% \rowcolor{lightgray}
% \multicolumn{3}{|c|}{\textbf{DNA source code encoding}}                                                   \\
\hline
% \rowcolor{lightgray}
{\textbf{Benchmark}} & {\textbf{Function name}} & {\textbf{$|$\textbf{CS}$|$}} \\ 
\hline
spmv ellpack & ellpack & 1600\\
\hline
bfs bulk & bulk &2352 \\
\hline
md knn & md\_kernel & 1600\\
\hline
viterbi & viterbi &  1152\\
\hline
gemm ncubed & gemm &  2744\\
gemm blocked & bbgemm  & 1600\\
\hline
fft strided & fft  & 64\\
\hline
\multirow{2}{*}{sort merge} & ms\_mergesort & 4096\\
& merge & 4096\\
\hline
stencil stencil2d & stencil & 1344\\
stencil stencil3d & stencil3d & 1536\\
\hline
\multirow{7}{*}{radix sort} & update & 2400 \\
& hist & 4704\\
& init & 484 \\
& sum\_scan  & 1280\\
& last\_step\_scan  & 800\\
& local\_scan &  704\\
& ss\_sort  & 1792 \\
\hline
\multirow{7}{*}{aes} & aes\_addRoundKey  &  500\\
& aes\_subBytes  & 50\\
& aes\_addRoundKey\_cpy  & 625\\
& aes\_shiftRows & 20\\
& aes\_mixColumns & 18 \\
& aes\_expandEncKey & 216 \\
& aes256\_encrypt\_ecb & 1944\\
\hline
\multirow{13}{*}{backprop} & get\_delta\_matrix\_weights1 & 21952 \\
& get\_delta\_matrix\_weights2 & 31213 \\ 
& get\_delta\_matrix\_weights3 & 21952 \\
& get\_oracle\_activations1  & 2401 \\
& get\_oracle\_activations2  & 1372 \\
& product\_with\_bias\_input\_layer & 1372\\
& product\_with\_bias\_second\_layer & 686\\
& product\_with\_bias\_output\_layer & 392\\
& backprop & 2048 \\
& add\_bias\_to\_activations  & 1372\\
& soft\_max  & 64\\
& take\_difference & 512\\
& update\_weights & 1024\\
\hline
\end{tabular}
% }
\label{tab:all}
\vskip -3em
\end{table}

\section{Available design space explorations}
\label{sec:data}

We provide a rich set of DSEs by targeting the benchmarks of the MachSuite collection of designs~\cite{reagen2014machsuite}. We have performed DSEs for 39 out of 50 functions in the benchmark suite, discarding those having a variable latency due to input-dependent control flows, and those having very small design spaces. The considered functions present on average 40 lines of code, with the biggest having 308 lines of code. 

For each design, we performed an extensive DSE across their configuration spaces -- the set of all possible implementation defined by the user -- up to tens of thousands of design points, these are reported in Table \ref{tab:all}.
%The description of the configuration space considered for each function can be retrieved from the database from the corresponding entry in the \emph{Configuration Space} table.
We used Vivado HLS~\cite{VivadoHLS} version 2018.2 to run syntheses with a target clock period of $10ns$ and targeting a ZynqMP Ultrascale+ (\texttt{\small xczu9eg}) FPGA chip.
We constrained the design spaces sizes by employing only power-of-two values for directives having a numerical range (e.g., loop-unrolling and array-partitioning factors). 
Moreover, in some DSEs we forced optimizations to have the same values, when intuitively such choice would lead to better cost/performance trade-offs (e.g., the partitioning factor of an array and the unrolling of a loop accessing it once every iteration).

Even when considering these constraints, the data collection required more than 4 years of single-core machine time. To speed up this process, GNU Parallel was adopted to collect synthesis data from up to 60 parallel instances of Vivado HLS, allowing us to populate the database in approximately 25 days of wall-clock time.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{imgs/ERD-crop.pdf}
\caption{\small Simplified scheme of the Entity-Relationship Diagram (ERD) of the DB4HLS syntheses database.}
\label{fig::erd}
\vskip -1em
\end{figure}

\section{DB4HLS infrastructure}
\label{sec:implementation}

In addition to the DSE data, the DB4HLS framework offers a) a database infrastructure hosting DSE in a structured and easy-to-access way, b) a domain-specific language used to describe a configuration space for a target design, c) an interface to generate new explorations and further enrich the database. The remaining of this section describes these further contributions in details.

\subsection{A database for DSEs}
\label{subsec:DB}

% The implemented Database, implemented in MySQL, comprises a description of the application targeted for exploration (upper part of Figure \ref{fig::erd}), and that of the explored HLS optimizations applied to each application (middle part of Figure \ref{fig::erd}). Finally, it reports the  resource and performance results obtained by synthesis (as described in the bottom part of the figure). Each of these components is described more in detail in the following paragraphs.

\begin{figure*}[t]
%\centering

\begin{minipage}{.48\textwidth}
  \centering
%  \vskip -2em
\begin{lstlisting}[caption={\texttt{last\_step\_scan} design (C code).}, label={code:last_step_scan} ,linewidth=\columnwidth,breaklines=true,language=C,
    firstnumber=1,
    numbers=left,
    stepnumber=1,
    numberblanklines=false,
    tabsize=1,
    basicstyle=\small,
    % basicstyle=\fontsize{8}{10}\ttfamily,
    breakatwhitespace=false,
    xleftmargin=2em]
void last_step_scan(int bucket[SIZE], int sum[RADIX]){
  int i, j, k;
  loop_1:for(i = 0; i < RADIX;i++){
    loop_2:for(j = 0; j < BLOCK; j++) {
      k = (i * BLOCK) + j;
      bucket[k] = bucket[k] + sum[i];
    }
  }
}
\end{lstlisting}
\end{minipage}
%
\hfill
\begin{minipage}{.48\textwidth}
%\vskip 0.5em
  \centering
\begin{lstlisting}[caption=Configuration Space of \texttt{last\_step\_scan}.,label={sweep:last_step_scan},linewidth=\columnwidth,breaklines=true,language=C,
    firstnumber=1,
    numbers=left,
    stepnumber=1,
    numberblanklines=false,
    tabsize=1,
    basicstyle=\small,
    % basicstyle=\fontsize{8}{10}\ttfamily,
    breakatwhitespace=false,
    xleftmargin=2em]
resource;last_step_scan;bucket;{RAM_2P_BRAM}
resource;last_step_scan;sum;{RAM_2P_BRAM}
array_partition;last_step_scan;bucket;1;{cyclic,block};{1->512,pow_2}
array_partition;last_step_scan;sum;1;{cyclic,block};{1->128,pow_2}@bind_a
unroll;last_step_scan;last_1;{1->128,pow_2}@bind_a
unroll;last_step_scan;last_2;{1,2,4,8,16}
clock;{10}
\end{lstlisting}
% \vskip -2em
\end{minipage}
% \vskip -2em
% \end{mdframed}
\vskip -1em
\caption{\small Left: Snippet of the \texttt{\small last\_step\_scan} C code function from MachSuite\cite{reagen2014machsuite}. The code was  rewritten  to  increase  readability,  without  modifying  its functionality. Right: An associated Configuration Space Descriptor (CSD). }\label{fig:mot_example}
\vskip -1.5em
\end{figure*}

The database structure, implemented in MySQL, comprises a description of the design targeted for exploration (top part of Figure \ref{fig::erd}), and that of the explored HLS optimizations applied to each design (middle part of Figure \ref{fig::erd}). Finally, it reports the resource and performance results obtained by synthesis (as described in the bottom part of the figure). Each of these components is described more in detail in the following.

Similarly to the taxonomy adopted in MachSuite \cite{reagen2014machsuite}, applications are identified by the \emph{benchmark} they belong to (e.g.: \texttt{aes}), by the \emph{algorithm} they realize (e.g.: \texttt{aes256\_encrypt}) and by the \emph{design} implementing such algorithms. As an example, two variants are provided by MachSuite for the \texttt{aes256\_encrypt} algorithm (one using lookup tables to store  encryption keys and one generating the values online), each corresponding to a separate design specified as C++ code.

A descriptor of the HLS optimizations considered for the DSEs are stored as entries in \emph{configuration space} table. Multiple explorations (hence, rows in the configuration space table) for the same design are possible, corresponding to different choices of optimizations, or explorations targeting different tools/FPGAs, or even contributions from different researchers. An entry in the \emph{configuration space} table is linked to many entries of the \emph{configuration} table, where each entry indicates a specific element of the design space.

A line in the \emph{configuration} table (that indicates the set of HLS optimizations defining a design space element) is linked to an entry in the \emph{implementation} table. Furthermore, the \emph{synthesis information} table provides additional information on each performed synthesis: the synthesis timestamp, the contributor that originated the data, the employed synthesis tool and version, and the targeted FPGA. Finally, each implementation links to one or more entries in the \emph{resources} and \emph{performance} tables, which report the synthesis outcomes. Resources are expressed as employed Flip-Flops, Look-Up Tables, Block RAMs (BRAM) and DSP blocks, while performances are reported in terms of effective latency.

%We created a database structure reflecting the terminology introduced in section \ref{sec:terminology}. In addition, we enhanced the notion of \emph{implementation} with the elements characterising it, such as the HLS tools generating it, and additional information regarding the synthesis process. 

%Figure \ref{fig::erd} represent a simplified Entity-Relationship Diagram (ERD) which describes the entities in the database and the inter-relationship, with the respective cardinalities, among them. 
%The upper part of the diagram highlights the relation among benchmark, application, algorithm, design, configuration space, implementation, and knob defined in Section \ref{sec:terminology}. 
%The bottom part of the diagram, depicts instead the relationship among a synthesis instance and the elements defining it. 
%While the upper part describes the elements defined before the DSEs from the user, the bottom half includes all the information generated during the exploration.

%\emph{Example}: Let's consider the \texttt{\small aes256\_encrypt} benchmark of \texttt{\small aes} from MachSuite. In this case  \texttt{\small aes} is the entry of the \emph{Benchmark} table. The \texttt{\small aes} application in the suite presents an \emph{algorithm} \texttt{\small aes256\_encrypt} which has two different designs: one using lookup tables to store the encryption keys (named \texttt{\small table}), and one generating the key online (named \texttt{\small no-table}). Both \texttt{\small table} and \texttt{\small no-table} are two different entries of the \emph{Design} table for \texttt{\small aes256\_encrypt} algorithm. Then, a configurations space for the \texttt{\small table} design, in the form of Configuration Space Descriptor (detailed in Section \ref{subsec:dsl}) is defined and stored in the \emph{Configuration space} table. Each of the associated configurations are stored in the \emph{Configuration} table and their knobs are entries of the \emph{Knob} table. The implementation associated to a configuration is stored in the \emph{Implementation} table, while the associated information about the synthesis tool and the machine running the synthesis in the \emph{HLS tool} and \emph{Machine} tables. Finally, the resulting performance, area and power results are stored in the \emph{Performance Result}, \emph{Area Result} and \emph{Power Result}, respectively.

\subsection{A domain-specific language for DSEs}\label{subsec:dsl}

Generating the different configurations associated with an DSE is a tedious and error-prone process when performed by hand. We therefore developed a Domain-Specific Language (DSL) to automatically and concisely define configuration spaces by employing Configuration Space Descriptors (CSDs). 

Each line of a descriptor encodes a \emph{knob}, which comprises a directive type, a label corresponding to its location in the design C/C++ code, and one or multiple sets of values. The number of sets is equal to the number of parameters required by the directive type. Values can be numerical when expressing optimizations such as loop unrolling or array partitioning factors, or categorical when determining the type of employed FPGA resources such as BRAM types.
A shorthand is provided for expressing regular value series (e.g., a succession of power-of-two values). Finally, we provide a \texttt{\small{@bind}} decorator, which constraints the values associated with different directives.
% forces two or more directives of a configuration to use the same associated directive value.

Figure \ref{fig:mot_example} shows for the function \texttt{\small last\_step\_scan} (Snippet \ref{code:last_step_scan}) an example of DSL defined to describe the configuration space defined for its DSE (Snippet~\ref{sweep:last_step_scan}).
The DSL defines seven different knobs. Line 1 of Snippet~\ref{sweep:last_step_scan} shows a knob with a single value: it associates a dual-ported BRAM to the array \texttt{\small bucket} that is the input of the function. Similarly, line 2 defines a dual-ported BRAM for the array \texttt{\small sum}.
Line 3 instead defines a knob governing the array\_partitioning directive defined by all the pairs having one of two partitioning strategies (\texttt{\small cyclic} and \texttt{\small block}) as the first component, and the ten possible partitioning factors  (all the powers of two from 1 up to 512) as the second one. The same is done in line 4, but defining a different set of partitioning factors (all the powers of two from 1 up to 128). 
Then line 5 and 6 define for \texttt{loop\_1} and \texttt{loop\_2} the associated set of unrolling factors to consider during the exploration, all the powers of two from 1 up to 128 and 16, respectively.
Both line 4 and 5 have a binding decorator (\texttt{\small @bind\_a}), that specifies that the array partitioning directive and the unrolling one must have the same partitioning and unrolling factor for all the configurations described by the CSD. 
Finally line 7 defines the target clock.

%\demo

The DSL generates the set of configurations of the design space as the Cartesian product of all knob values: $CS = K_{1} \times K_{2} \times \dots \times K_{N}$;
% \begin{equation}
% CS = K_{1} \times K_{2} \times \dots \times K_{N}
% \end{equation}
where  $N$ is the number of considered knobs, and $K_{i}$ is the set of values related to each $i$ knob, i.e. the set of values that the directive associated to the knob $i$ can assume,
taking into account the restrictions imposed by the \texttt{bind} decorator. For a directive  with  multiple parameters, $K_{i}$ is itself the Cartesian product among each set of values.
The size of the configuration space is then given by its cardinality ($|CS|$).

The configuration space descriptor of Figure \ref{fig:mot_example} in Snippet \ref{sweep:last_step_scan} describes a configuration space with 1600 different configurations. Without the binding decorator, the cardinality of the configuration space would be 12800.

\subsection{A framework for parallelizing HLS runs}

Figure \ref{fig::infrastructure} gives a high-level view of the infrastructure, realized through Bash and Python scripts, which we provide to automate DSE and commit their outcomes in DB4HLS. Starting from a user-provided design and Configuration Space Descriptor (CSD), configuration files are automatically generated and stored in the database. Then, using GNU Parallel \cite{gnuparallel}, a tunable number of instances of an employed HLS tool (we use Vivado HLS for the data collection described in Section \ref{sec:data}) are concurrently and independently executed, one for each configuration. As synthesis runs terminate, the retrieved performance and resources information are also stored in DB4HLS, and new HLS processes are launched until all configurations have been explored. 

MySQL statements can then be used to retrieve data from the tables in the database and to access the design's implementations and the associated performance and resources results.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{imgs/infrastructure.pdf}
\caption{\small Adding DSE to DB4HLS with parallel processing.}
\label{fig::infrastructure}
\vskip -1.5em
\end{figure}

\section{Case Study}

Herein, we showcase two possible uses of DB4HLS. We use the database both to compare the results of two DSE methodologies, and as a source of knowledge for one of them. We employed a lattice-based strategy (LB) from \cite{ferretti2018lattice}, and one leveraging prior knowledge (PK)\cite{Ferretti20Oct}, to perform DSEs for the \texttt{\small local\_scan} design space available in DB4HLS.
Figure \ref{fig:exploration} reports the Pareto curve obtained by LB and PK for the \texttt{\small local\_scan} design space. Grey dots represent the area and latency of the 704 implementations belonging to the \texttt{\small local\_scan} design space provided by DB4HLS. The figure also reports the approximated Pareto fronts retrieved by the lattice methodology described in \cite{ferretti2018lattice} (LB) and by the prior-knowledge strategy in \cite{Ferretti20Oct} (PK).
% In this example the database has a double role. It is used both to allow a direct comparison among two different methodologies and as initial source of knowledge for the PK one. 

In this scenario, DB4HLS is employed to comparatively evaluate the two strategies, without requiring to re-run ex-novo a large number of time-consuming synthesis runs. Moreover, in the case of PK, the database mandates the availability of a set of \emph{source} design spaces in order to extract previous knowledge. In fact, DB4HLS can be effectively employed in these cases, or in similar ML-based methods \cite{wang20Mar}, to provide the required knowledge base. 

\begin{figure}[t]
\centering
% \begin{minipage}{.5\linewidth}
  \centering
%   \captionsetup{justification=centering,margin=2mm}
  \captionsetup{margin=1mm}
  \includegraphics[width=\linewidth]{imgs/comparison-crop.pdf}
% \end{minipage}%
% % \begin{minipage}{.5\linewidth}
%   \centering
% \captionsetup{margin=1mm}
%   \includegraphics[width=\linewidth]{imgs/bad-AEsim.pdf}
% \end{minipage}
%  \caption{\small Grey dots represent the area and latency of the 704 implementations belonging to the \texttt{\small local\_scan} design space provided by DB4HLS. The figure also reports the approximate Pareto fronts retrieved by the lattice methodology described in \cite{ferretti2018lattice} (LB) and by the prior-knowledge strategy in \cite{Ferretti20Oct} (PK).}
 \caption{\small Example of DSEs comparison employing DB4HLS.}\label{fig:exploration}
%  both to allow a direct comparison among two different methodologies (LB \cite{ferretti2018lattice} and PK \cite{Ferretti20Oct}) and as initial source of knowledge for PK. }\label{fig:exploration}
% \vspace{-5mm}
\vskip -1.5em
\end{figure}


\section{Conclusions}

DB4HLS offers an extensive set of DSEs targeting functions from MachSuite \cite{reagen2014machsuite}. The data collection is made publicly available and will be will be updated increasing the number of design explorations and targeted benchmarks. In addition, further design spaces can be effectively defined through a novel domain-specific language and a framework to efficiently contribute novel explorations to DB4HLS. Both the DB4HLS database and the framework for DSE generation are publicly available at \small{\texttt{https://www.inf.usi.ch/phd/ferretti/db4hls.html}}. 

% \vskip -2em

%To the best of our knowledge, this is the first attempt make publicly available a database of HW implementations which can help researchers both in the standardisation process of methodologies evaluation and boosting ML-oriented research in the field. We aim at constantly improve and update the database gathering a more various and extensive set of implementations targeting other benchmark suite from the state-of-the-art.
%aiming at helping to satisfy the need of data required by such methodologies.

